MonoGAE: Roadside Monocular 3D Object Detection with Ground-Aware Embeddings

Although the majority of recent autonomous driving systems concentrate on developing perception methods based on ego-vehicle sensors, there is an overlooked alternative approach that involves leveraging intelligent roadside cameras to help extend the ego-vehicle perception ability beyond the visual range. We discover that most existing monocular 3D object detectors rely on the ego-vehicle prior assumption that the optical axis of the camera is parallel to the ground. However, the roadside camera is installed on a pole with a pitched angle, which makes the existing methods not optimal for roadside scenes. In this paper, we introduce a novel framework for Roadside Monocular 3D object detection with ground-aware embeddings, named MonoGAE. Specifically, the ground plane is a stable and strong prior knowledge due to the fixed installation of cameras in roadside scenarios. In order to reduce the domain gap between the ground geometry information and high-dimensional image features, we employ a supervised training paradigm with a ground plane to predict high-dimensional ground-aware embeddings. These embeddings are subsequently integrated with image features through cross-attention mechanisms. Furthermore, to improve the detector's robustness to the divergences in cameras' installation poses, we replace the ground plane depth map with a novel pixel-level refined ground plane equation map. Our approach demonstrates a substantial performance advantage over all previous monocular 3D object detectors on widely recognized 3D detection benchmarks for roadside cameras. The code and pre-trained models will be released soon.

==> authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{{authors/LeiYang.jpg}}}]{Lei Yang} was born in DaTong, Shanxi Province, China in 1993. He received his B.E. degree from Taiyuan University of Technology, Taiyuan, China,
and the M.S. degree from the Robotics Institute at Beihang University, in 2018. Then he joined the Autonomous Driving R$\&$D Department of JD.COM as an algorithm researcher from 2018 to 2020. He is now a Ph.D. student in the School of Vehicle and Mobility at Tsinghua University since 2020.

His current research interests include computer vision, 3D scene understanding and autonomous driving.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{{authors/JiaxinYu.jpg}}}]{Jiaxin Yu} was born in Nanchong, Sichuan Province China in 2000. She received her B.E. degree from Chongqing Jiaotong University, Chongqing, China. She is now a M.S. student in the School of Civil Engineering and Transportation at South China University of Technology since 2021.     Her current research interests include object detection and 3D scene understanding.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in, clip,keepaspectratio]{{authors/XinyuZhang.png}}}]{Xinyu Zhang} was born in Huining, Gansu Province, and he received a B.E. degree from the School of Vehicle and Mobility at Tsinghua University, in 2001. 

He was a visiting scholar at the University of Cambridge. He is currently a researcher with the School of Vehicle and Mobility, and the head of the Mengshi Intelligent Vehicle Team at Tsinghua University.

Dr. Zhang is the author of more than 30 SCI/EI articles. His research interests include intelligent driving and multimodal information fusion.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{{authors/JunLi.jpg}}}]{Jun Li} was born in Jilin Province, China in 1958. He received a Ph.D. degree in internal-combustion engineering at Jilin University of Technology, in 1989. 

He has joined the China FAW Group Corporation in 1989 and currently works as a professor with the School of Vehicle and Mobility at Tsinghua University. Now he also serves as the chairman of the China Society of Automotive Engineers (SAE). 
In these years, Dr. Li has presided over the product development and technological innovation of large-scale automobile companies in China. Dr. Li has many scientific research achievements in the fields of automotive powertrains, new energy vehicles, and intelligent connected vehicles. 

Dr. Li is the author of more than 98 papers. In 2013, Dr. Li was awarded an academician of Chinese Academy of Engineering (CAE) for contributions to vehicle engineering. 
\end{IEEEbiography}

	
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{{authors/LiWang.png}}}]{Li Wang} was born in Shangqiu, Henan Province, China in 1990. He received his Ph.D. degree in mechatronic engineering at State Key Laboratory of Robotics and Systems, Harbin Institute of Technology, in 2020. 
He was a visiting scholar at Nanyang Technology of University for two years. Currently, he is a postdoctoral fellow in the State Key Laboratory of Automotive Safety and Energy, and the School of Vehicle and Mobility, Tsinghua University.

Dr. Wang is the author of more than 15 SCI/EI articles. His research interests include autonomous driving perception, 3D robot vision and multi-modal fusion.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{{authors/YiHuang.png}}}]
{Yi Huang} joined R\&D Center of the Chinese FAW group as a vehicle engineer from 2009 to 2018. He is now a PhD student in the School of Vehicle and Mobility at Tsinghua University since 2021. His research interests are autonomous driving and e Ammonia-hydrogen fuel for heavy-duty vehicles.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{{authors/ChuangZhang.jpg}}}]
{Chuang Zhang} received the B.E. degree from Southeast University, Nanjing, China, in 2017, and the M.S. from Beihang University, Beijing, China, in 2020. He is currently a Ph.D. student in mechanical engineering with the School of Vehicle and Mobility, Tsinghua University. His research interests include object detection, multi-object tracking and multi-sensor fusion.
\end{IEEEbiography}


==> table/alg.tex <==
\begin{algorithm}[h!t]
\caption{Refined ground plane equation map generator}
\label{alg:algorithm}
\textbf{Parameters Definition}: \\
    $P$: the position $(x,y,z)$ of objects on the ground.\\
    $O$: the pixel $(u,v)$ that are obtained by projecting the $P$.\\
    $K$: the camera's intrinsic matrix. \\ 
    $N$: the number of objects on the ground. \\
    $denorms$: a pixel-level fine-grained ground plane equation map, each pixel is assigned the parameters $\alpha$, $\beta$, $\gamma$, and $d$ of the initial ground plane equation $G_{initial}$.\\
    $findRecent()$: the purpose of this function is to divide an input set of points into multiple groups, with each group containing three points, where the covered area by the three points is as small as possible, and there is no overlap between the groups. Please refer to \cite{kramer2013k}.\\ 
    $getEquation()$: this function can obtain the equation of the plane determined by three input points. Please refer to formula(\ref{eq6}).\\
    $inArea()$: this function can determine whether the input pixel $(i,j)$ is in the triangular region formed by the input three points. If it is, it returns True.\\
    
\vspace{-0.2cm}
\hrule
\vspace{0.1cm}
\textbf{Input}: \\
$P = \left\{p_1, ...,p_N\right\}$\\
$denorms \in \mathbb{R}^{h\times w \times 4}$\\
\textbf{Output}: \\
    $denorms'$ is a refined pixel-level ground equation map.\\
\textbf{Begin:}
\begin{algorithmic}[1] %[1] enables line numbers
\STATE $denorms'   =  denorms$
\STATE $multiGroups = findRecent(P)$\\
\FOR {$group$ in $multiGroups$}
 \STATE $\left\{p_1,p_2,p_3\right\} \gets group$\\
 \STATE $G_{revised} = getEquation(p_1,p_2,p_3)$\\
 \STATE $\left\{\alpha', \beta', \gamma', d'\right\} \gets 
 G_{revised}$\\
 \FOR {$n$ in $(1,2,3)$}
  \STATE $x, y, z \gets p_n$\\
  \STATE $[u, v, 1]^T = K  [x/z, y/z, 1]^T$\\
  \STATE $o_n= \left\{u,v\right\}$\\
 \ENDFOR
 \FOR {$i,j$ in $zip(range(h),range(w))$}
 % \FOR {$i$ in $range(h)$}
 %  \FOR {$j$ in $range(w)$}
  \IF{$inArea(o_{1}, o_{2}, o_{3}, i, j)$}
   \STATE $denorms'[i,j] = \left\{\alpha',\beta', \gamma', d'\right\}$\\
  \ENDIF
  % \ENDFOR
 \ENDFOR\\
\ENDFOR\\
\STATE \textbf{return} $denorms'$\\
\end{algorithmic}
\textbf{End}
\end{algorithm}
